A Survey on Edge Performance Benchmarking

Edge computing is the next Internet frontier that will leverage computing resources located near users, sensors, and data stores to provide more responsive services. Therefore, it is envisioned that a large-scale, geographically dispersed, and resource-rich distributed system will emerge and play a key role in the future Internet. However, given the loosely coupled nature of such complex systems, their operational conditions are expected to change significantly over time. In this context, the performance characteristics of such systems will need to be captured rapidly, which is referred to as performance benchmarking, for application deployment, resource orchestration, and adaptive decision-making. Edge performance benchmarking is a nascent research avenue that has started gaining momentum over the past five years. This article first reviews articles published over the past three decades to trace the history of performance benchmarking from tightly coupled to loosely coupled systems. It then systematically classifies previous research to identify the system under test, techniques analyzed, and benchmark runtime in edge performance benchmarking.

==> discussion.tex <==
In this paper, we have discussed a range of existing papers and Internet sources related to edge performance benchmarking. In this discussion, we focused on implicit and explicit benchmarks, where explicit benchmarks are defined as papers or Internet sources that focus on providing a tangible contribution to the field of benchmarking. We not only discussed edge benchmarking sources, but we also considered a broader perspective by examining benchmarking papers from closely related fields such as clouds or grids that could be adapted for use or reused directly in the context of edge environments. Implicit benchmarks can typically be found in the evaluation sections of systems papers for edge computing. Although they do not focus on providing a novel contribution to the field of benchmarking, they often use novel workloads and measurement approaches that could serve as inspiration for future explicit benchmarking papers in this field. Therefore, we cannot and do not claim completeness for our selected set of implicit benchmarks because the body of work on edge computing (including closely related topics such as fog computing and mobile edge computing) is too extensive to cover in a single survey paper. Additionally, explicit benchmarks can be identified objectively, but whether or not a paper qualifies as an implicit benchmark is highly subjective. Based on careful analysis and discussion by the authors, we feel confident that the set of selected implicit benchmarks, while not necessarily complete, contains no false positives. Overall, we strongly believe that even a limited subset of implicit benchmarks adds significant value to this survey and to the emerging field of edge performance benchmarking.



In this paper, we also focused on the performance of edge platforms and systems. However, in addition to performance, there are other quality dimensions such as elastic scalability, data consistency, security and privacy, and availability, that typically exhibit direct or indirect tradeoff relationships~\cite{diss_bermbach,book_cloud_service_benchmarking}. We are not aware of any \emph{edge} benchmarking approaches for evaluating these other quality dimensions. Again, we believe that benchmarking approaches from other closely related domains, such as cloud computing, can often be adapted or reused for edge environments. Regarding elastic scalability, the discussions presented in~\cite{rabl2012solving,back-34,back-40,binnig2009weather,islam2012elasticity,paper_kuhlenkamp_bench_elasticy} can serve as a starting point. Similar starting points can be identified for availability~\cite{paper_bermbach_benchmarking_web_apis,paper_bermbach_webapibenchmarking2,shao2009user,toeroe2012service,hauer2020meaningful,fox1999harvest,paper_klems_consistency_benchmarking}, data consistency~\cite{paper_zellag_consistency_benchmarking,paper_wada_consistency_monitoring,paper_golab_analyzing_consistency,paper_anderson_consistency_measurements,back-36,back-38,paper_bermbach_consistency,diss_bermbach}, and security and privacy~\cite{back-46,paper_pallas_et_al_sac_2017_evidence_based,paper_pallas_security_performance_hbase,bermbach2019benchmarking,apostolopoulos1999transport,kant2000architectural,coarfa2006performance,shastri2019understanding}. A detailed discussion of these other quality dimensions is beyond the scope of this paper.


==> quality.tex <==
As already discussed, benchmarking is the process of stressing a system while observing its response to a range of quality metrics.
%\footnote{Where not indicated otherwise, this section is based on~\cite{book_cloud_service_benchmarking}.}. 
In this, benchmarking captures non-functional properties or ``how well'' a given system can fulfill its functional properties. In the context of non-functional properties, there are three concepts which need to be considered: quality indicators, quality metrics, and quality tradeoffs. In this section, we present an overview of these three concepts along with examples of quality indicators for edge benchmarking.

\subsection{Quality Indicators}
There is a broad range of different quality indicators that can be further divided into sub-qualities.
%, i.e., quality can be structured as a tree. 
For instance, performance as a quality indicator can be broken down into its two qualities: throughput -- amount of load a system can handle, and latency -- time to process a single or batch request~\cite{book_cloud_service_benchmarking}.

Most quality indicators describe a deviation from an ideal state which is usually unreachable. For example, latency can never be zero and availability can (on a long time horizon) never be ``always''. Throughput as a counter example, may be zero but its ideal state is ``infinity'', which is also an unreachable (ideal) state. It is also important to distinguish between a measurement of the ideal state and the system operating at that ideal state. When the measurement resolution is low, it may be possible to measure, for example, a latency of zero, but the actual system will have a latency that is negligible, but greater than a zero value. Overall, this means that quality indicators are usually bounded in at least one direction -- they either have an upper or lower limit~\cite{book_cloud_service_benchmarking}.

\subsection{Quality Metrics}
To measure quality, a quality metric which is a function that maps a concrete quality level to a specific value and a unit is required. ``A quality metric is, therefore, the function that expresses differences in quality''~\cite{book_cloud_service_benchmarking}; for each quality metric that has to be observed, there may be more than one such function. 

There are atleast nine requirements that quality metrics need to fulfill~\cite{paper_kaner_software_quality_metrics,book_cloud_service_benchmarking,diss_bermbach}:
(1)~\textit{Correlation}: There needs to be a (preferably linear) correlation between the quality indicator under observation and the metric output, i.e., ``changes in quality behavior should always be visible in metric output''~\cite{book_cloud_service_benchmarking}.
(2)~\textit{Tracking}: When a quality level changes, the metric output should change and do so (preferably) instantly.
(3)~\textit{Monotonicity}: When a quality level changes in a particular direction then the metric output should always change in the same direction, no matter what the quality level was at the start or at the end. In other words, increasing a quality may either increase or decrease the metric output but must do so consistently for all quality levels.
(4)~\textit{Discriminative Power}: ``The metric should be able to clearly differentiate between low and high quality levels''~\cite{book_cloud_service_benchmarking}.
(5)~\textit{Reproducibility}: Aside from measurement errors, a repeated measurement should always yield the same metric output for an unchanged quality level as long as the experiment setup is not changed~\cite{paper_bermbach_benchmarking_middleware}.
(6)~\textit{Resolution}: A metric needs to have a large set of metric output values and should preferably be continuous to differentiate between arbitrary small differences in quality level. This also implies that metrics should usually not be aggregates but should rather ``report raw, single values that can be aggregated in a second phase based on standard aggregation methods''~\cite{book_cloud_service_benchmarking}.
(7)~\textit{Granularity}: A metric should only measure a single quality indicator at a time. Otherwise, changes in one quality may offset changes in another.
(8)~\textit{Meaningfulness}: "A metric may have a (specific) target audience but there must be at least one target audience for which the (metric outputs) are meaningful and understandable...(so) that they can actually use them for their purposes''~\cite{book_cloud_service_benchmarking}.
(9)~\textit{Reliability}: The above requirements should be fulfilled ``for at least P\% of the application of the metric''~\cite{paper_kaner_software_quality_metrics}. Concrete values for P depend on the specific use case but should be as high as possible, preferably 100\%.

%\begin{enumerate}
%    \item Correlation: There needs to be a (preferably linear) correlation between the quality indicator under observation and the metric output, i.e., ``changes in quality behavior should always be visible in metric output''~\cite{book_cloud_service_benchmarking}.
%    \item Tracking: When a quality level changes, the metric output should change and do so (preferably) instantly.
%    \item Monotonicity: When a quality level changes in a particular direction then the metric output should always change in the same direction, no matter what the quality level was at the start or at the end. In other words, increasing a quality may either increase or decrease the metric output but must do so consistently for all quality levels.
%    \item Discriminative Power: ``The metric should be able to clearly differentiate between low and high quality levels''~\cite{book_cloud_service_benchmarking}.
%    \item Reproducibility: Aside from measurement errors, a repeated measurement should always yield the same metric output for an unchanged quality level as long as the experiment setup is not changed~\cite{paper_bermbach_benchmarking_middleware}.
%    \item Resolution: A metric needs to have a large set of metric output values and should preferably be continuous to differentiate between arbitrary small differences in quality level. This also implies that metrics should usually not be aggregates but should rather ``report raw, single values that can be aggregated in a second phase based on standard aggregation methods''~\cite{book_cloud_service_benchmarking}.
%   \item Granularity: A metric should only measure a single quality indicator at a time. Otherwise, changes in one quality may offset changes in another.
%    \item Meaningfulness: "A metric may have a (specific) target audience but there must be at least one target audience for which the (metric outputs) are meaningful and understandable...(so) that they can actually use them for their purposes''~\cite{book_cloud_service_benchmarking}.
%    \item Reliability: The above requirements should be fulfilled ``for at least P\% of the application of the metric''~\cite{paper_kaner_software_quality_metrics}. Concrete values for P depend on the specific use case but should be as high as possible, preferably 100\%.
%\end{enumerate}

To develop a measurement method in edge benchmarking, quality metrics that fulfill these requirements as much as possible (sometimes, there are constraints which make it hard to fulfill them completely) are required. In most cases, such a metric already hints how it can be measured. For instance, response time (as a performance metric for latency) is usually measured by noting the timestamp before sending a request and upon receipt of the response. Then the duration between both is calculated and reported as the metric value.

\subsection{Examples of Quality Indicators}

There is a wide range of different quality indicators - those that are omnipresent, such as performance or availability, those that are relevant to a class of systems, for example, data consistency for systems replicating state, and those than can only be observed indirectly, such as elastic scalability. In this section, an overview of a selected set of quality indicators (shown in Figure~\ref{fig:quality-qualityindicators}) and their relevance to edge benchmarking is discussed. The indicators considered are not comprehensive, but only a subset is chosen for discussion in this paper. 

\begin{wrapfigure}{l}{0.48\textwidth}
%\begin{figure}
  \centering
  \includegraphics[width=0.49\textwidth]{images/quality-qualityindicators.png}
  \caption{An overview of a subset of quality indicators relevant to edge benchmarking}
  \label{fig:quality-qualityindicators}
%\end{figure}
\end{wrapfigure}

\subsubsection{Performance}
Performance is an omnipresent, directly observable quality indicator and is broken down into the two quality dimensions throughput and latency. \textit{Throughput} generally describes the amount of load a system can simultaneously handle, while \textit{latency} describes the time necessary to handle unit load. For a system that is accessed in a request-response manner, throughput is usually measured as requests per second (potentially as maximum throughput while not violating SLAs, such as latency) where as latency is measured as the time between sending a request and receiving a response.

In the context of edge benchmarking, performance is an important quality indicator for a number of reasons. First, resources at the edge are usually hardware limited. The capability to handle as many requests in parallel (throughput) and to service a single request as fast as possible (latency) will directly affect how rapidly requests will need to be offloaded from the edge to the cloud~\cite{paper_bermbach_auctions4function_placement}. This has an impact on latency for requests originating from latency-critical applications. Second, most edge computing use cases have latency concerns that are alleviated by placing a few components or services of a system at the edge to reach QoS goals. An example is interconnected or autonomous driving where a delayed response leads to a degradation of the service.

Most TPC\footnote{\url{www.tpc.org}} and SPEC\footnote{\url{www.spec.org}} benchmarks are performance benchmarks. Benchmark approaches quantify performance of relational database systems~\cite{back-45}, NoSQL stores~\cite{back-23,back-41,back-37}, VMs~\cite{back-39,scheuner:14-cloudcom,scheuner:19-icpe-tutorial,Lenk:2011}, block storage~\cite{paper_kuhlenkamp_aisle_service_level_pressure}, or serverless Function-as-a-Service (FaaS) platforms~\cite{paper_kuhlenkamp_benchmarking_faas_ccp,paper_kuhlenkamp_faas_foundation,lloyd2018serverless}. They can also be used in continuous integration processes to avoid performance degradation of software systems~\cite{van2012kieker,grambow_continuous_benchmarking:_2019}.

\subsubsection{Elastic Scalability}
Elastic scalability is omnipresent in that it is relevant to all systems but is generally not directly observable. However, a less elasticly scalable system is observable through performance degradation. Elastic scalability can be broken down into the qualities scalability and elasticity. \textit{Scalability} describes how well a system adapts to changes based on available resources, which is how much load can be handled, for example, when doubling the available resources (ideally, at least twice the load).
When a system is scaled out by adding more machines or using a bigger machine (and correspondingly scaled up), the new ``load'' state is not reached instantaneously. Instead, there is an intermediate period during which neither the previous nor the new load level is reached. While this may be a gradual change for some systems, others may experience a significant performance drop (for example, when large data chunks need to be redistributed across machines). \textit{Elasticity} describes what happens in between the previous and the new stable state, how long it takes to reach the stable state and how severely performance is impacted during scaling. 

In the context of edge benchmarking, elastic scalability has applicability in multiple scenarios. First, during on-demand federation with local peer nodes to increase capacity (scaling out).
%less important than performance on the edge since scaling a system at the edge will rarely be possible (aside from on-demand federation with nearby peer nodes) due to the limits of available resources. 
Second, during offloading operations when an application component is moved across multiple edge, intermediary, or cloud resources, the application will need to adapt to the underlying infrastructure (scaling up or down). The assessment whether a system under test follows a design that supports this, is a key goal when benchmarking applications that can move between edge and cloud~\cite{paper_bermbach_fog_vision}.

There are a number of benchmarking approaches that quantify elastic scalability. For example, metrics for measuring scalability of cloud database systems have been defined~\cite{back-40,binnig2009weather}, scalability experiments have been carried out~\cite{rabl2012solving,back-34}, generic cloud elasticity metrics have been defined~\cite{islam2012elasticity}, and elasticity of serverless FaaS platforms has been benchmarked~\cite{paper_kuhlenkamp_bench_elasticy}.


\subsubsection{Availability}
Availability is an omnipresent quality that is relevant to all types of systems and can be directly observed. It is directly related to fault-tolerance (availability in the presence of failures) and reliability. Availability is understood to define whether a system  responds to requests. However, it can be challenging to determine which of the following conditions meet the criteria for availability. Is a system available (i) when the host can be reached, (ii) when the host returns any response, or (iii) when the host returns a correct response?~\cite{paper_bermbach_benchmarking_web_apis}. 
In addition to considering individual requests, availability can be aggregated to \textit{uptime} of an entire service. This is based on \textit{mean time between failures} (how often a failure occurs), and \textit{mean time to repair} (how long a service remains unavailable upon a failure)~\cite{shao2009user,toeroe2012service}. 
Recently, \textit{windowed user-uptime} has been proposed as a more meaningful (and aggregated) availability metric~\cite{hauer2020meaningful}. 
%An alternative metric, specifically covering the relation to data consistency has been proposed by Fox and Brewer~\cite{fox1999harvest}. 
%Their metrics harvest and yield respectively describe the likelihood of getting \emph{some} response or getting a \emph{complete} response and have been used to study the availability and consistency behavior of messaging services~\cite{paper_klems_consistency_benchmarking}.

In the context of edge benchmarking, availability is relevant for large scale edge resource deployments to understand aggregated failure statistics across a large number of small distributed machines that are connected through unreliable networks. Fault-tolerance and the resulting degree of degradation is often more important than uptime for edge-based applications raising the questions -- how well does the system deal with failures and how many failures can the fault-tolerance mechanisms cope with?

\subsubsection{Security and Privacy}
Security and privacy are fundamental and required by design, unless a system is running in an entirely isolated environment. Privacy refers to the individual's rights to control of their own personal data is multi-faceted, across concepts of consent management~\cite{UlbrichtYaPPLLightweightPrivacy2018} or data minimization~\cite{paper_pallas_fog4privacy}. It is usually governed by legislation such as the General Data Protection Regulation (GDPR). Security, on the other hand, is about avoiding any misuse of a system and associated data. Security cannot be completely benchmarked as this would require knowledge of \emph{all} possible attacks on a system, but it can be approximated using all \emph{known} attacks. Security benchmarks consider preferences of providers~\cite{bermbach2019benchmarking} or performance overheads of security mechanisms (for example, of database systems~\cite{back-46,paper_pallas_et_al_sac_2017_evidence_based,paper_pallas_security_performance_hbase}, homomorphic encryption~\cite{paper_pallas_grambow_three_tales_disillusion}, web servers~\cite{apostolopoulos1999transport,kant2000architectural,coarfa2006performance}, and SOAP messaging~\cite{shirasuna2004performance}). The only benchmarking approach on privacy that the authors are aware of evaluates the effects of GDPR compliance on database workloads~\cite{shastri2019understanding}.

In the context of edge benchmarking, novel security mechanisms using entirely new attack vectors need to be explored, since physical access to an edge device are a possibility, which is nearly impossible with cloud resources embedded within data center distant from consumers~\cite{paper_bermbach_fog_vision}. Nonetheless, edge resources can improve privacy, e.g., by separating data lakes~\cite{paper_pallas_fog4privacy}. %Alongside novel security and privacy techniques, we will have to develop new benchmarking approaches and measurement techniques for edge environments.


\subsubsection{Data Consistency}
Data consistency is not necessarily an omnipresent quality as it only matters to systems managing data. %Such systems, however, are needed in almost any application so that data consistency is nevertheless highly relevant. Data consistency related problems with data consistency can easily become directly visible to applications -- this, however, depends on the way in which applications interact with the data management system. Data consistency is probably the only quality which can achieve its perfect level ("strict consistency"). System developers, however, tend to sacrifice consistency in favor of improved latency and availability, particularly in the presence of failures.
Data consistency has two dimensions, ordering and staleness, which can be considered from a client and a provider perspective~\cite{book_cloud_service_benchmarking}. Usually, the client perspective is taken, which is more relevant for benchmarking as it describes the effects directly visible to a benchmarking client. \textit{Staleness} occurs when an update becomes (partially) visible before executing on all replicas. In this sense, applications then read outdated data. Staleness, however, can in many cases be tolerated by applications~\cite{paper_vogels_eventually_consistent}. \textit{Ordering} from a provider perspective describes the degree to which requests can be executed in a different order on different replicas. From a client perspective, such ordering issues become visible as violations of monotonic reads, monotonic writes, read your writes, and write follows reads~\cite{paper_bermbach_consistency}. Violations of these guarantees from an underlying datastore can either become visible to end users or make the application development quite challenging. For instance, violations of monotonic writes imply that writing and then updating some value is not guaranteed to result in the updated value on all replicas. There are multiple benchmarking approaches that consider data consistency~\cite{paper_zellag_consistency_benchmarking,paper_wada_consistency_monitoring,paper_golab_analyzing_consistency,paper_anderson_consistency_measurements,back-36,back-38}.

In the context of edge benchmarking, data consistency as a quality is only relevant when considering multi-node deployments, for example, across several edge nodes or when integrating the edge and cloud. In these scenarios, consistency guarantees are affected by inter-node latency of replicas (tends to be large) when replicas are deployed on edge nodes. Furthermore, design choices of the replica synchronization protocols in LAN and WAN deployments for edge systems need to be analyzed through experimental evaluation. Additional data related challenges that should be considered by edge benchmarks have been reported in~\cite{dataconsistency-bv-01}. 


\subsection{Quality Tradeoffs}
The quality indicators considered above are rarely isolated; instead, they usually have a direct or indirect tradeoff relationship~\cite{diss_bermbach,book_cloud_service_benchmarking}. A direct tradeoff relationship between two qualities A and B implies that increasing A is likely to decrease B. Indirect relationships are transitive. For example, direct tradeoffs between qualities A and B as well as B and C mean that an increase of A reduces B, which may be offset by a decrease in C instead. There are a wide range of direct tradeoffs, such as the CAP theorem\footnote{\url{http://www.cs.berkeley.edu/~brewer/cs262b-2004/PODC-keynote.pdf}} and the PACELC model~\cite{paper_abadi_pacelc}, which describe tradeoffs between \textit{data consistency and latency} as well as data consistency and availability (in the presence of failures). Other known direct tradeoffs are between \textit{performance and cost} (adding more infrastructure resources increases cost) or \textit{security and performance} (additional efforts for encryption or authentication schemes introduce an overhead and hence a performance degradation).

Benchmarking should carefully analyze the quality of interest for tradeoff relationships and measure both sides of the tradeoff~\cite{book_cloud_service_benchmarking}. The same holds for edge benchmarking. For example, consider performance benchmarks for a distributed storage system deployed across multiple geo-distributed edge nodes. System A replicates updates synchronously across all replicas, system B replicates updates asynchronously. Any performance benchmark is likely to identify system B as the superior system. This changes when a data consistency benchmark is run in addition and both quality indicators are weighed against each other.

==> systemundertest-table-ch.tex <==

\begin{table}
\revision{
\centering
\footnotesize
\begin{tabular}{|p{7.5cm}|p{0.3cm}|p{0.3cm}|p{0.3cm}|p{0.3cm}|p{0.8cm}|p{0.5cm}|}
\hline
\multirow{3}{*}{} & \multicolumn{4}{c|}{\textbf{Optimization}} & \multicolumn{2}{c|}{\textbf{Deployment}}  \\
 & \multicolumn{4}{c|}{\textbf{options}} & \multicolumn{2}{c|}{\textbf{options}}  \\
\cline{2-7}
\textbf{Techniques analyzed by edge performance benchmarks} & \begin{sideways}\textbf{Energy consumption}~\end{sideways} & \begin{sideways}\textbf{Monetary cost}\end{sideways} & \begin{sideways}\textbf{Quality-of-Service}\end{sideways} &
\begin{sideways}\textbf{Hardware utilization}\end{sideways} &
\begin{sideways}\textbf{Offloading}\end{sideways}  &
\begin{sideways}\textbf{Virtualization}\end{sideways}\\ 
\hline
CoAP benchmark~\cite{eb-01}, HERMIT~\cite{eb-10} 
 & N & N & Y & Y  & N & N\\
\hline
Virt. benchmark~\cite{eb-02}
& N & N & N & Y & N & V, C \\
\hline
Virt. benchmark~\cite{eb-03} &  Y & N & Y & Y  & N & C \\
\hline
Voice benchmark~\cite{eb-04} &  N &  N &  Y &  N  & D $\xrightarrow[]{}$ E & N \\
\hline
RIoTBench~\cite{eb-05} &  N &  N & Y &  Y  & N & V \\
\hline
TPCx-IoT &  N &  Y & Y &  N  & N & N \\
\hline
D-Cube~\cite{eb-06} &  Y &  N &  Y &  N  & N & N \\
\hline
 CAVBench~\cite{eb-07} &  N &  N &  Y &  Y  & N & N\\
\hline
EdgeBench~\cite{eb-08} &  N &  N & Y &  Y  & E $\xrightarrow[]{}$ C & V, C \\
\hline
 Edge AIBench~\cite{eb-09} &  N &  N & N &  N  & N & N \\
\hline
LEAF~\cite{eb-11}, AIoTBench~\cite{eb-12} &  N &  N & N &  N  & N & N \\
\hline
pCAMP~\cite{eb-13} &  Y &  N & Y &  N  & N & N \\
\hline
DeFog~\cite{intro-07} &  N &  N & Y &  N  & C $\xrightarrow[]{}$ E & V, C \\
\hline
Edgedroid~\cite{eb-15} &  N &  N & Y &  N  & N & C \\
\hline
MAVBench~\cite{eb-16} &  Y &  N & Y &  N  & D $\xrightarrow[]{}$ C & N \\ \hline
IoTBench~\cite{eb-17} &  Y &  N & N &  N  & N & N \\ \hline
SoftwarePilot &  N &  N & N &  N  & N & V, C \\ \hline
Machine learning accelerator benchmark~\cite{eb-18} & Y &  N & N &  Y & N & V \\ \hline
Edge FPGA-based Neural Net benchmark~\cite{eb-19} & Y &  N & Y &  N  & N & N \\ \hline
\end{tabular}
\caption{\revision{Comparison of the characteristics of the techniques analyzed by explicit edge performance benchmarks; Offloading: End-user \textbf{D}evice, \textbf{E}dge, \textbf{C}loud, or \textbf{N}one; Virtualization: \textbf{V}irtual machine, \textbf{C}ontainer, or \textbf{N}one};}
\label{tab:techniquesanalysed-existing_benchmark}
}
\end{table}




\begin{table}
\centering
\footnotesize
\begin{tabular}{|p{8.5cm}|p{0.3cm}|p{0.3cm}|p{0.3cm}|p{0.3cm}|p{0.9cm}|p{0.5cm}|}
\hline
\multirow{3}{*}{} & \multicolumn{4}{c|}{\textbf{Optimization}} & \multicolumn{2}{c|}{\textbf{Deployment}}  \\
 & \multicolumn{4}{c|}{\textbf{options}} & \multicolumn{2}{c|}{\textbf{options}}  \\
\cline{2-7}
\textbf{Techniques analyzed by edge performance benchmarks} & \begin{sideways}\textbf{Energy consumption}~\end{sideways} & \begin{sideways}\textbf{Monetary cost}\end{sideways} & \begin{sideways}\textbf{Quality-of-Service}\end{sideways} 
& \begin{sideways}\textbf{Hardware utilization}\end{sideways}
& 
\begin{sideways}\textbf{Offloading}\end{sideways} & \begin{sideways}\textbf{Virtualization}\end{sideways}\\ 
\hline
Resource allocation benchmark~\cite{ta-02}, MECO benchmark~\cite{ta-01}, RTLBB~\cite{ta-03}, EEDOA~\cite{ta-05}
%, Offloading~\cite{ta-43} 
& \multirow{2}{*}{Y} & \multirow{2}{*}{N} & \multirow{2}{*}{N} & \multirow{2}{*}{N} &  \multirow{2}{*}{$D\xrightarrow[]{}E$} & \multirow{2}{*}{N}\\
\hline
MIMO benchmark~\cite{ta-68} & \multirow{1}{*}{Y} & \multirow{1}{*}{N} & \multirow{1}{*}{N} & \multirow{1}{*}{N} &  \multirow{1}{*}{$D\xrightarrow[]{}C$} & \multirow{1}{*}{N}\\
\hline
%Service placement~\cite{ta-26, ta-39,ta-44,ta-22},
IoT benchmark~\cite{ta-26}, LBVS~\cite{ta-22}, MeFoRE~\cite{ta-28}, 
%FogTorch~\cite{ta-45}, Scheduling~\cite{ta-23}, 
VEC benchmark~\cite{ta-31} & \multirow{1}{*}{N} & \multirow{1}{*}{N} &  \multirow{1}{*}{Y} & \multirow{1}{*}{N} &
\multirow{1}{*}{$D\xrightarrow[]{}E$} & \multirow{1}{*}{N}  \\
\hline
%ITEM~\cite{ta-34}, 
%Service placement~\cite{ta-40,ta-42} & 
IoT benchmark~\cite{ta-40} & \multirow{1}{*}{N} & \multirow{1}{*}{Y} & \multirow{1}{*}{Y} & \multirow{1}{*}{N} &  \multirow{1}{*}{$D\xrightarrow[]{}E$} & \multirow{1}{*}{N} \\
\hline
%Service placement~\cite{ta-19} &  \multirow{1}{*}{N} & \multirow{1}{*}{Y} & \multirow{1}{*}{Y} & \multirow{1}{*}{N} &  \multirow{1}{*}{$C\xrightarrow[]{}E$} & \multirow{1}{*}{N} \\ \hline
DYVERSE~\cite{intro-09}, ENORM~\cite{intro-08} &  \multirow{1}{*}{N} &  \multirow{1}{*}{N} &  \multirow{1}{*}{Y} &  \multirow{1}{*}{N} &   \multirow{1}{*}{$C\xrightarrow[]{}E$} &  \multirow{1}{*}{V, C} \\
\hline
ECC benchmark~\cite{ta-35} &  N &  Y & Y &  N &  $D\xrightarrow[]{}E$ &  N \\
\hline
%Resource allocation~\cite{ta-06,ta-08}
%Resource allocation benchmark~\cite{ta-06}
%&  N &  Y & N &  N  & $D\xrightarrow[]{}E$  &  N\\
%\hline
%Resource allocation~\cite{ta-17} &  Y &  Y &  N &  N  & N &  N \\ \hline
%JCORAO~\cite{ta-09} &  Y &  Y &  N &  N  &  $D\xrightarrow[]{}E$ &  N \\ \hline
%Resource allocation~\cite{ta-24}, Application placement~\cite{ta-11} &  Y &  Y &  N & N  &  $C\xrightarrow[]{}E$ &  N \\ \hline
%HMAOA~\cite{ta-12}, Offloading~\cite{ta-63} &  Y &  N &  Y &  N  &  $D\xrightarrow[]{}E$ &  N \\ \hline
%Offloading~\cite{ta-58,ta-49} &  Y &  N &  Y &  N  &  $D\xrightarrow[]{}C$ &  N \\ \hline
YEAST~\cite{ta-61}, EDAL~\cite{ta-60} &  Y &  N &  Y &  N  &  N &  N \\
\hline
Content delivery benchmark~\cite{ta-50} &  N &  N & Y &  Y & N &  N \\
\hline
%Data replication~\cite{ta-53} &  N &  N & Y &  N & N &  N \\ \hline
Cloudlet benchmark~\cite{ta-51} &  N &  N & N &  N  & $C\xrightarrow[]{}E$  &  V \\
\hline
%FocusStack~\cite{ta-59} &  N &  N &  N &  N &  N  &  C \\ \hline
%ParaDrop~\cite{ta-64} &  N &  N &  N &  Y & $D\xrightarrow[]{}E$  &  C \\ \hline
Migration benchmark~\cite{ta-67} &  N &  N & Y &  N  &  $E\xrightarrow[]{}E$ &  C \\
\hline
Cloudlet benchmark~\cite{ta-69} &  Y &  N & Y &  N  & $D\xrightarrow[]{}E$  &  N \\
\hline
Virt. benchmark~\cite{eb-03} &  Y &  N & N &  Y &  N &  C \\
\hline
\end{tabular}
\caption{Comparison of the characteristics of the techniques analyzed by explicit edge performance benchmarks; Offloading: End-user \textbf{D}evice, \textbf{E}dge, \textbf{C}loud, or \textbf{N}one;  Virtualization: \textbf{V}irtual machine, \textbf{C}ontainer, \textbf{N}one}
\label{tab:techniquesanalysed}
\end{table}

%\begin{table}
%\centering
%\footnotesize
%\begin{tabular}{|p{7.5cm}|p{0.3cm}|p{0.3cm}|p{0.3cm}|p{0.3cm}|p{0.8cm}|p{0.9cm}|p{0.5cm}|}
%\hline
%\multirow{3}{*}{} & \multicolumn{4}{c|}{\textbf{Optimization}} & \multicolumn{3}{c|}{\textbf{Deployment}}  \\
% & \multicolumn{4}{c|}{\textbf{options}} & \multicolumn{3}{c|}{\textbf{options}}  \\
%\cline{2-8}
%\textbf{Techniques analyzed by edge performance benchmarks} & \begin{sideways}\textbf{Energy consumption}~\end{sideways} & \begin{sideways}\textbf{Monetary cost}\end{sideways} & \begin{sideways}\textbf{Quality-of-Service}\end{sideways} 
%& \begin{sideways}\textbf{Hardware utilization}\end{sideways}
%& 
%\begin{sideways}\textbf{Platforms}\end{sideways} & \begin{sideways}\textbf{Offloading}\end{sideways} & \begin{sideways}\textbf{Virtualization}\end{sideways}\\ 
%\hline
%Resource allocation~\cite{ta-01, ta-02}, RTLBB~\cite{ta-03}, EEDOA~\cite{ta-05}, Offloading~\cite{ta-43} & \multirow{2}{*}{Y} & \multirow{2}{*}{N} & \multirow{2}{*}{N} & \multirow{2}{*}{N} & \multirow{2}{*}{S} & \multirow{2}{*}{$D\xrightarrow[]{}E$} & \multirow{2}{*}{N}\\
%\hline
%Resource allocation~\cite{ta-68} & \multirow{1}{*}{Y} & \multirow{1}{*}{N} & \multirow{1}{*}{N} & \multirow{1}{*}{N} & \multirow{1}{*}{S} & \multirow{1}{*}{$D\xrightarrow[]{}C$} & \multirow{1}{*}{N}\\
%\hline
%Service placement~\cite{ta-26, ta-39,ta-44,ta-22}, MeFoRE~\cite{ta-28}, FogTorch~\cite{ta-45}, Scheduling~\cite{ta-23}, Offloading~\cite{ta-31} & \multirow{2}{*}{N} & \multirow{2}{*}{N} &  \multirow{2}{*}{Y} & \multirow{2}{*}{N} &
%\multirow{2}{*}{S} &  \multirow{2}{*}{$D\xrightarrow[]{}E$} & \multirow{2}{*}{N}  \\
%\hline
%ITEM~\cite{ta-34}, Service placement~\cite{ta-40,ta-42} &  \multirow{1}{*}{N} & \multirow{1}{*}{Y} & \multirow{1}{*}{Y} & \multirow{1}{*}{N} & \multirow{1}{*}{S} & \multirow{1}{*}{$D\xrightarrow[]{}E$} & \multirow{1}{*}{N} \\
%\hline
%Service placement~\cite{ta-19} &  \multirow{1}{*}{N} & \multirow{1}{*}{Y} & \multirow{1}{*}{Y} & \multirow{1}{*}{N} & \multirow{1}{*}{S} & \multirow{1}{*}{$C\xrightarrow[]{}E$} & \multirow{1}{*}{N} \\
%\hline
%DYVERSE~\cite{intro-09}, ENORM~\cite{intro-08} &  \multirow{1}{*}{N} &  \multirow{1}{*}{N} &  \multirow{1}{*}{Y} &  \multirow{1}{*}{N} &  \multirow{1}{*}{D, E, C} &  \multirow{1}{*}{$C\xrightarrow[]{}E$} &  \multirow{1}{*}{V, C} \\
%\hline
%Service migration~\cite{ta-35} &  N &  Y & Y &  N &  D, E &  $D\xrightarrow[]{}E$ &  N \\
%\hline
%Resource allocation~\cite{ta-06,ta-08} &  N &  Y & N &  N &  S & $D\xrightarrow[]{}E$  &  N\\
%\hline
%Resource allocation~\cite{ta-17} &  Y &  Y &  N &  N &  S & N &  N \\
%\hline
%JCORAO~\cite{ta-09} &  Y &  Y &  N &  N &  S &  $D\xrightarrow[]{}E$ &  N \\
%\hline
%Resource allocation~\cite{ta-24}, Application placement~\cite{ta-11} &  Y &  Y &  N & N &  S &  $C\xrightarrow[]{}E$ &  N \\
%\hline
%HMAOA~\cite{ta-12}, Offloading~\cite{ta-63} &  Y &  N &  Y &  N &  S &  $D\xrightarrow[]{}E$ &  N \\
%\hline
%Offloading~\cite{ta-58,ta-49} &  Y &  N &  Y &  N &  S &  $D\xrightarrow[]{}C$ &  N \\
%\hline
%YEAST~\cite{ta-61}, EDAL~\cite{ta-60} &  Y &  N &  Y &  N &  S &  N &  N \\
%\hline
%Data replication~\cite{ta-50} &  N &  N & Y &  Y &  E &  N &  N \\
%\hline
%Data replication~\cite{ta-53} &  N &  N & Y &  N &  D, E &  N &  N \\
%\hline
%Wearable cognitive assistance~\cite{ta-51} &  N &  N & N &  N &  D, E, C & $C\xrightarrow[]{}E$  &  V \\
%\hline
%FocusStack~\cite{ta-59} &  N &  N &  N &  N &  D, E, C & N  &  C \\
%\hline
%ParaDrop~\cite{ta-64} &  N &  N &  N &  Y &  D, E, C & $D\xrightarrow[]{}E$  &  C \\
%\hline
%Migration~\cite{ta-67} &  N &  N & Y &  N &  E &  $E\xrightarrow[]{}E$ &  C \\
%\hline
%Offloading~\cite{ta-69} &  Y &  N & Y &  N &  D, E, C & $D\xrightarrow[]{}E$  &  N \\
%\hline
%Virtualization~\cite{eb-03} &  Y &  N & N &  Y &  E &  N &  C \\
%\hline
%\end{tabular}
%\caption{Comparing the characteristics of techniques analyzed in edge performance benchmarks; Offloading: End-user \textbf{D}evice, \textbf{E}dge, \textbf{C}loud, or \textbf{N}one;  Virtualization: \textbf{V}irtual machine, \textbf{C}ontainer, \textbf{N}one}
%\label{tab:techniquesanalysed}
%\end{table}


%\begin{landscape}
%\begin{table}
%\centering
%\footnotesize
%\begin{tabular}{|p{4cm}|p{1.5cm}|p{1cm}|c|p{1.1cm}|p{1cm}|p{1cm}|p{1.1cm}|p{3cm}|}
%\begin{tabular}{|p{4cm}|p{0.3cm}|p{0.3cm}|p{0.3}|p{0.3cm}|p{0.3cm}|p{0.3cm}|p{0.3cm}|p{0.3cm}|}
%\hline
%\multirow{3}{*}{} & \multicolumn{3}{c|}{\textbf{Optimization}} & \multicolumn{5}{c|}{\textbf{Deployment}}  \\
% & \multicolumn{3}{c|}{\textbf{criteria}} & \multicolumn{5}{c|}{\textbf{options}}  \\
%\cline{2-9}
%\textbf{Techniques Analyzed by edge performance benchmarking} & \begin{sideways}\textbf{Energy consumption}~\end{sideways} & \begin{sideways}\textbf{Monetary cost}\end{sideways} & \begin{sideways}\textbf{Quality-of-Service}\end{sideways} & \begin{sideways}\textbf{End-user device}\end{sideways} & \begin{sideways}\textbf{Edge}\end{sideways} & \begin{sideways}\textbf{Cloud}\end{sideways} & \begin{sideways}\textbf{Simulated platform}\end{sideways} & \begin{sideways}\textbf{Virtualization}\end{sideways}\\ 
%\hline
%Resource allocation~\cite{ta-01, ta-02,ta-68} \newline RTLBB~\cite{ta-03} \newline EEDOA~\cite{ta-05} \newline Offloading~\cite{ta-43} & \multirow{4}{*}{Y} & \multirow{4}{*}{N} & \multirow{4}{*}{N} & \multirow{4}{*}{N} & \multirow{4}{*}{N} & \multirow{4}{*}{N} & \multirow{4}{*}{Y} & \multirow{4}{*}{N}\\
%\hline
%Service placement~\cite{ta-26, ta-39,ta-44,ta-22} \newline MeFoRE~\cite{ta-28} \newline FogTorch~\cite{ta-45} \newline Scheduling~\cite{ta-23} \newline Offloading~\cite{ta-31} & \multirow{5}{*}{N} & \multirow{5}{*}{N} &  \multirow{5}{*}{Y} & \multirow{5}{*}{N} & \multirow{5}{*}{N} & \multirow{5}{*}{N} & \multirow{5}{*}{Y} & \multirow{5}{*}{N}  \\
%\hline
%ITEM~\cite{ta-34} \newline Service placement~\cite{ta-40,ta-42,ta-19} &  \multirow{2}{*}{N} & \multirow{2}{*}{Y} & \multirow{2}{*}{Y} & \multirow{2}{*}{N} & \multirow{2}{*}{N} & \multirow{2}{*}{N} & \multirow{2}{*}{Y} & \multirow{2}{*}{N} \\
%\hline
%DYVERSE~\cite{intro-09} \newline ENORM~\cite{intro-08} &  \multirow{2}{*}{N} &  \multirow{2}{*}{N} &  \multirow{2}{*}{Y} &  \multirow{2}{*}{Y} &  \multirow{2}{*}{Y} &  \multirow{2}{*}{Y} &  \multirow{2}{*}{N} &  \multirow{2}{*}{C} \\
%\hline
%Service migration~\cite{ta-35} &  N &  Y & Y &  Y &  Y &  N &  N &  N \\
%\hline
%Resource allocation~\cite{ta-06,ta-08} &  N &  Y & N &  N &  N &  N &  Y &  N \\
%\hline
%Resource allocation~\cite{ta-17, ta-24} \newline JCORAO~\cite{ta-09} \newline Application placement~\cite{ta-11} &  \multirow{3}{*}{Y} &  \multirow{3}{*}{Y} &  \multirow{3}{*}{N} &  \multirow{3}{*}{N} &  \multirow{3}{*}{N} &  \multirow{3}{*}{N} &  \multirow{3}{*}{Y} &  \multirow{3}{*}{N} \\
%\hline
%HMAOA~\cite{ta-12} \newline Offloading~\cite{ta-58, ta-49,ta-63} \newline YEAST~\cite{ta-61} \newline EDAL~\cite{ta-60} &  \multirow{4}{*}{Y} &  \multirow{4}{*}{N} &  \multirow{4}{*}{Y} &  \multirow{4}{*}{N} &  \multirow{4}{*}{N} &  \multirow{4}{*}{N} &  \multirow{4}{*}{Y} &  \multirow{4}{*}{N} \\
%\hline
%Data replication~\cite{ta-50} &  N &  N & Y &  N &  Y &  N &  N &  N \\
%\hline
%Data replication~\cite{ta-53} &  N &  N & Y &  Y &  Y &  N &  N &  N \\
%\hline
%Wearable cognitive assistance~\cite{ta-51} &  N &  N & N &  Y &  Y &  Y &  N &  V \\
%\hline
%FocusStack~\cite{ta-59} \newline ParaDrop~\cite{ta-64} &  \multirow{2}{*}{N} &  \multirow{2}{*}{N} &  \multirow{2}{*}{N} &  \multirow{2}{*}{Y} &  \multirow{2}{*}{Y} &  \multirow{2}{*}{Y} &  \multirow{2}{*}{N} &  \multirow{2}{*}{C} \\
%\hline
%Migration~\cite{ta-67} &  N &  N & Y &  N &  Y &  N &  N &  C \\
%\hline
%Offloading~\cite{ta-69} &  Y &  N & Y &  Y &  Y &  Y &  N &  N \\
%\hline
%Virtualization~\cite{eb-03} &  Y &  N & N &  N &  Y &  N &  N &  C \\
%\hline
%\end{tabular}
%\caption{Comparing the characteristics of techniques analyzed in edge performance benchmarks; Virtualization: \textbf{V}irtual machine, \textbf{C}ontainer, or \textbf{N}one}
%\label{tab:techniquesanalysed}
%\end{table}
%\end{landscape}



